Indirect Measurement of Hepatic Drug Clearance by Fitting Dynamical Models

We present an indirect signal processing-based measurement method for biological quantities in humans that cannot be directly measured. We develop the method by focusing on estimating hepatic enzyme and drug transporter activity through breath-biopsy samples clinically obtained via the erythromycin breath test (EBT): a small dose of radio-labeled drug is injected and the subsequent content of radio-labeled CO$_2$ is measured repeatedly in exhaled breath; the resulting time series is analyzed. To model EBT we developed a 14-variable non-linear reduced order dynamical model that describes the behavior of the drug and its metabolites in the human body well enough to capture all biological phenomena of interest. Based on this system of coupled non-linear ordinary differential equations (ODEs) we treat the measurement problem as inverse problem: we estimate the ODE parameters of individual patients from the measured EBT time series. These estimates then provide a measurement of the liver activity of interest. The parameters are hard to estimate as the ODEs are stiff and the problem needs to be regularized to ensure stable convergence. We develop a formal operator framework to capture and treat the specific non-linearities present, and perform perturbation analysis to establish properties of the estimation procedure and its solution. Development of the method required 150,000 CPU hours at a supercomputing center, and a single production run takes CPU 24 hours. We introduce and analyze the method in the context of future precision dosing of drugs for vulnerable patients (e.g., oncology, nephrology, or pediatrics) to eventually ensure efficacy and avoid toxicity.

==> Shared_iPBPKR.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{ntheorem}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

\newenvironment{noinds_itemize}{\begin{list}{$\bullet$}
{\setlength{\rightmargin}{0em} \setlength{\leftmargin}{1.2em}
\setlength{\itemsep}{0em} \setlength{\topsep}{0em}
\setlength{\parsep}{0em}}}{\end{list}}


% Prevent itemized lists from running into the left margin inside theorems and proofs
\usepackage{enumitem}
\setlist[enumerate]{leftmargin=.5in}
\setlist[itemize]{leftmargin=.5in}

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
%\newsiamremark{remark}{Remark}
%\newsiamremark{hypothesis}{Hypothesis}
%\crefname{hypothesis}{Hypothesis}{Hypotheses}
%\newsiamthm{claim}{Claim}


% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{iPBPK-R Modeling: Indirect Measurement of In vivo Activities of Drug Metabolism and Transport}



%% Authors: full names plus addresses.
%\author{Yoko Franchetti\thanks{Department of Pharmaceutical Sciences, Center of Clinical Pharmaceutical Sciences, University of Pittsburgh School of Pharmacy, Pittsburgh, PA
%  (\email{yof8@pitt.edu}).}
%\and Thomas D. Nolin\thanks{Department of Pharmacy and Therapeutics, Center of Clinical Pharmaceutical Sciences, University of Pittsburgh School of Pharmacy, Pittsburgh, PA
%  (\email{nolin@pitt.edu}).}
%\and Franz Franchetti\footnotemark[3]\thanks{Department of Electrical and Computer Engineering, Carnegie Mellon University, Pittsburgh, PA}
%(\email{franzf@andrew.cmu.edu}).
%}
%%

% author names and IEEE memberships
% note positions of commas and nonbreaking spaces ( ~ ) LaTeX will not break
% a structure at a ~ so this keeps an author's name from being broken across
% two lines.
% use \thanks{} to gain access to the first footnote area
% a separate \thanks must be used for each paragraph as LaTeX2e's \thanks
% was not built to handle multiple paragraphs
%

\author{Yoko Franchetti,
        Thomas D. Nolin,
        and~Franz~Franchetti,~\IEEEmembership{Senior Member,~IEEE}% <-this % stops a space
\thanks{Yoko Franchetti was with the Department of Pharmaceutical Sciences, Center of Clinical Pharmaceutical Sciences, University of Pittsburgh School of Pharmacy, Pittsburgh, PA, USA e-mail: yof8@pitt.edu.}%
\thanks{Thomas D. Nolin was with the Department of Pharmacy and Therapeutics, Center of Clinical Pharmaceutical Sciences, University of Pittsburgh School of Pharmacy, Pittsburgh, PA, USA e-mail nolin@pitt.edu.}%
\thanks{Franz Franchetti was with the Department of Electrical and Computer Engineering, Carnegie Mellon University, Pittsburgh, PA, USA email franzf@andrew.cmu.edu.}%
\thanks{Manuscript received XXX YY, 2020; revised XXX YY, 2020.}}

% note the % following the last \IEEEmembership and also \thanks -
% these prevent an unwanted space from occurring between the last author name
% and the end of the author line. i.e., if you had this:
%
% \author{....lastname \thanks{...} \thanks{...} }
%                     ^------------^------------^----Do not want these spaces!
%
% a space would be appended to the last name and could cause every name on that
% line to be shifted left slightly. This is one of those "LaTeX things". For
% instance, "\textbf{A} \textbf{B}" will typeset as "A B" not "AB". To get
% "AB" then you have to do: "\textbf{A}\textbf{B}"
% \thanks is no different in this regard, so shield the last } of each \thanks
% that ends a line with a % and do not let a space in before the next \thanks.
% Spaces after \IEEEmembership other than the last one are OK (and needed) as
% you are supposed to have spaces between the names. For what it is worth,
% this is a minor point as most people would not even notice if the said evil
% space somehow managed to creep in.


% The paper headers
\markboth{Transactions on Biomedical Engineering,~Vol.~X, No.~Y, August~20XX}%
{Franchetti \MakeLowercase{\textit{et al.}}: Individualized Physiologically Based Pharmacokinetic Modeling of Rate Data (iPBPK-R)}
% The only time the second header will appear is for the odd numbered pages
% after the title page when using the twoside option.
%
% *** Note that you probably will NOT want to include the author's ***
% *** name in the headers of peer review papers.                   ***
% You can use \ifCLASSOPTIONpeerreview for conditional compilation here if
% you desire.





\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}

\newcommand\comment[1]{}
\newcommand\mypar[1]{{\bf #1.}}
%\newcommand\comment[1]{#1}
%%% Local Variables:
%%% mode:latex
%%% TeX-master: "Article_iPBPKR"
%%% End:

